Nonparametric Masked Language Modeling

Existing language models (LMs) predict tokens with a softmax over a finite vocabulary, which can make it difficult to predict rare tokens or phrases. We introduce NPM, the first nonparametric masked language model that replaces this softmax with a nonparametric distribution over every phrase in a reference corpus. NPM fills in the [MASK] solely from retrieving a token from a text corpus. We show that NPM can be efficiently trained with a contrastive objective and an in-batch approximation to full corpus retrieval. Zero-shot evaluation on 16 tasks including classification, fact probing and question answering demonstrates that NPM outperforms significantly larger parametric models, either with or without a retrieve-and-generate approach. It is particularly better at dealing with rare patterns (word senses or facts) and predicting rare or nearly unseen words (e.g., non-Latin script). We release the model and code at github.com/facebookresearch/NPM.

==> sections/03-method.tex <==
\begin{figure*}[t]
\centering \footnotesize
\resizebox{2\columnwidth}{!}{\includegraphics{imgs/npm-training.png}}\vspace{-.3em}
\caption{
The high-level idea of training \ours\ (Section~\ref{subsubsec:ours-train}).
\textcolor{orange}{\textbf{\mask}} indicates the masked token whose target token is {\em Seahawks}. %
\textcolor{myred}{Positives} are tokens from other sequences in-batch that share the vocab
(in the \mytextbox{myred}{red box}),
and \textcolor{myblue}{negatives} are tokens from other sequences in-batch that are not positives (in the (in the \mytextbox{myblue}{blue box}).
%
We maximize the similarity scores between the masked token and positives, and minimize the similarity scores between the masked token and negatives.
%
In practice, the batch includes many masked tokens, although the figure only shows one.
%
}\label{fig:training}
\end{figure*}

\sewon{This describes single-token version first.}


We first describe \ours\ which retrieves a token from the corpus to fill in the \mask\ (Section~\ref{subsec:ours}). We then describe \oursmulti, an extension of \ours\ that offers an infinite output space by retrieving an \ngram\ (Section~\ref{subsec:ours-multi}).

\subsection{\ours}\label{subsec:ours}

We introduce \ours, the first \textbf{N}on\textbf{\textsc{p}}arametric \textbf{M}asked Language Model.
\ours\ consists of the encoder and a reference corpus $\mathcal{C}$, and models a \np\ distribution over a reference corpus (Figure~\ref{fig:intro}).
The key idea is to map all the text in the corpus into a dense vector space using the encoder, and when given a query with a \mask\ at inference, use the encoder to locate the nearest token from the corpus and fill in the \mask.

We first describe inference of \ours\ assuming a learned encoder (Section~\ref{subsubsec:ours-inference}), and then describe how we train the encoder to map the text into a good vector space (Section~\ref{subsubsec:ours-train}).

% \sewon{I debated between describing training first and then inference vs. describing inference first and then training. I ended describing inference first, because inference is easier to understand, and a lot of choices in training can be seen as efforts to make training as close as possible to inference.}


\subsubsection{\ours: Inference}\label{subsubsec:ours-inference}

The encoder maps every distinct token in a reference corpus $\mathcal{C}$ into a dense vector space.
At test time, the encoder maps the masked query into the same vector space and retrieves tokens from $\mathcal{C}$ to fill in the \mask. 
Here, $\mathcal{C}$ does not have to be the same as the training corpus, and can be replaced or scaled at test time without training the encoder.

Formally, given a reference corpus with $N$ tokens in total: $\mathcal{C} = \{c_1, \cdots, c_N \}$,
we construct $N$ number of $h$-dimensional vectors $\mathbf{c}_1, \cdots, \mathbf{c}_N \in \mathbb{R}^h$ by feeding the text into the encoder.

At inference time, given a query whose $t$-th token is \mask: $q_1...q_{t-1}, \mask, q_{t+1}...q_L$, we feed it into the encoder:$$\mathbf{q}_1...\mathbf{q}_L = \mathrm{Encoder}(q_1...q_{t-1}, \mask, q_{t+1}...q_L).$$ We then take $\mathbf{q}_t$ as a vector that represents the \mask\ token in the query.
%
Finally, the prediction is made by aggregating the similarity scores to the tokens in $\mathcal{C}$:$$\argmax_{v \in \mathcal{V}} \sum_{i=1}^N \mathbb{I}[c_i=v] \mathrm{exp}(\mathrm{sim}(\mathbf{q}_t, \mathbf{c}_i)),$$where 
$\mathrm{sim}(\cdot,\cdot): \mathbb{R}^h \times \mathbb{R}^h \xrightarrow{} \mathbb{R}$ is a pre-defined similarity function
%$\mathrm{sim}(\cdot,\cdot)$ is a similarity function used at training time,
and $\mathcal{V}$ is the vocabulary set.

In practice, since computing scores over all tokens in $\mathcal{C}$ is infeasible, an approximation is made by computing scores for the top $k$ nearest neighbors only, and treating other tokens to have a similarity score of $-\mathrm{Inf}$. More precisely, indices of the tokens$$i^1,i^2,\cdots,i^k=\argtopk_i\mathrm{sim}(\mathbf{q}_t, \mathbf{c}_i)$$ are obtained by using an index (e.g., FAISS~\citep{johnson2019billion}), and the following is returned as a prediction:$$\argmax_{v \in \mathcal{V}} \sum_{i \in \{i^1...i^k\}} \mathbb{I}[c_i=v] \mathrm{exp}(\mathrm{sim}(\mathbf{q}_t, \mathbf{c}_i)).
$$

%We note that our inference largely follows the \knn\ inference from \citet{khandelwal2020generalization}, but with an adaptation to make it work with masked LMs instead of casual LMs.

\vspace{-.2em}
\paragraph{Similarity function.}
The choice of similarity function can be flexible. We follow \citet{zhong2022training} in using a scaled inner product:$$\mathrm{sim}(\mathbf{h}_1,\mathbf{h}_2)=\frac{\mathbf{h}_1 \cdot \mathbf{h}_2}{\sqrt{h}}.$$

\subsubsection{\ours: Training}\label{subsubsec:ours-train}

\ours\ is trained to ensure that the encoder maps the text into a good dense vector space.
%
We train \ours\ on a large, unlabeled text corpus using a self-supervised, contrastive objective~\citep{oord2018representation}.
%
We use an in-batch approximation by defining positive and negatives within the batch, removing the need for keeping and updating the retrieval index during training~\citep{wu2020scalable}.


We illustrate the key idea first, and then describe the training objective and how masked tokens are chosen.

\begin{figure*}[t]
\centering \footnotesize
\resizebox{2.05\columnwidth}{!}{\includegraphics{imgs/masking.png}}\vspace{-.3em}
\caption{
Comparison of different masking strategies.
For simplicity, this figure assumes the number of sequences in the batch is 2. Spans to mask out are chosen based on whether there is any co-occurring spans in other sequences in the batch. Then, \ours\ replaces each token in the span with a \mask\ (Section~\ref{subsubsec:ours-train}), and \oursmulti\ replaces the whole span with \mask\mask\ (Section~\ref{subsubsec:ours-train-multi}).
}\label{fig:masking}
\end{figure*}

\vspace{-.2em}
\paragraph{Key idea with an example.}
In Figure~\ref{fig:training}, the \textcolor{orange}{\textbf{\mask}} corresponds to {\em Seahawks}.
The model should retrieve other tokens from a reference corpus that are {\em Seattle} when the model is given a query like this at test time.

We train the model to do so by approximating the full corpus to the other sequences in the batch.
%
Specifically, we encourage the vector corresponding to \mask\ (\textcolor{orange}{$\blacksquare$})
to be closer to the vectors of the tokens in the batch that are {\em Seahawks} (\textcolor{myred}{$\blacksquare$}), and to be distant from vectors of the other tokens in the batch which are not {\em Seahawks} (\textcolor{myblue}{$\blacksquare$}).
%
In this way, we can encourage the model to retrieve {\em Seattle} from a reference corpus when it is given a sequence with a \mask\ that is supposed to be {\em Seattle} at test time.
%

\vspace{-.2em}
\paragraph{Objective.} Formally, let $x_1...x_L$ be a sequence of tokens, whose subset is replaced with \mask\ and converted to $\hat{x}_1...\hat{x}_L$. % be the same sequence, a subset of which replaced with \mask.
%
Both the masked sequence and the unmasked sequence are fed into the encoder, and each token is mapped into an $h$-dimensional vector $\mathbf{x}_i$ or $\mathbf{\hat{x}}_i$.
\begin{eqnarray*}\mathbf{x}_1...\mathbf{x}_L&=&\mathrm{Encoder}(x_1...x_L), \\
\mathbf{\hat{x}}_1...\mathbf{\hat{x}}_L&=&\mathrm{Encoder}(\hat{x}_1...\hat{x}_L).\end{eqnarray*}
The training objective is then defined as:$$
    \sum_{t=1}^L \mathbb{I}[\hat{x}_t=\mask]l(x_t,\hat{x}_t),
$$ where $l(x_t,\hat{x}_t)$ is $$-\mathrm{log}\frac{
        \sum_{\mathbf{y} \in \mathcal{Y}^+(x_t)} \mathrm{exp}(\mathrm{sim}(\mathbf{\hat{x}}_t, \mathbf{y}))
    }{
        \sum_{\mathbf{y} \in \mathcal{Y}^+(x_t) \cup \mathcal{Y}^-(x_t)} \mathrm{exp}(\mathrm{sim}(\mathbf{\hat{x}}_t, \mathbf{y}))
    }.
$$


Here,
$\mathrm{sim}(\cdot,\cdot)$ is a similarity function defined in Section~\ref{subsubsec:ours-inference},
and $\mathcal{Y}^+(x_t)$ and $\mathcal{Y}^-(x_t)$ are sets of vectors corresponding to {\em positives} and {\em negatives} of $x_t$, respectively, which we detail in the next paragraph.
%
Note that this objective resembles the contrastive learning objectives in prior work~\citep{mikolov2013distributed,oord2018representation,chen2020simple,karpukhin2020dense} with an extension that allows {\em multiple} positives.


\vspace{-.2em}
\paragraph{In-batch positives and negatives.}
Positives and negatives are defined as a function of the batch. They are a set of tokens from {\em other} sequences in the batch that share (or do not share) the vocab.
%
Formally, let $B = {x^1...x^B}$ be a batch of $B$ sequences, where $x^i$ is a sequence of tokens $x^i_1...x^i_L$. Then, positives and negatives of $x^i_t$ are as follows:\begin{eqnarray*}
    \mathcal{Y}^+(x^i_t)&=&\left\{ x^j_m | x^i_t = x^j_m \text{~and~} i \neq j\right\}, \\
    \mathcal{Y}^-(x^i_t)&=&\left\{ x^j_m | x^i_t \neq x^j_m \text{~and~} i \neq j\right\}.
\end{eqnarray*}
The size of the batch is important for effective training. We were able to use large batch by gathering all sequences from multiple GPUs used in training.

\vspace{-.2em}
\paragraph{Masking.}
Before training, we need to mask out a subset of tokens from a batch of sequences.
One possible choice is uniform masking, which independently determines whether or not to mask out each token~\citep{devlin2019bert,liu2019roberta}.
We instead use span masking~\citep{joshi-etal-2017-triviaqa}, which masks spans (consecutive tokens) whose length is sampled from a geometric distribution.
Different from previous work, all masked tokens (or spans) are guaranteed to co-occur in the other sequences in the batch, so that there is at least one positive found in the batch.
For instance, in an example in Figure~\ref{fig:masking},
%In uniform masking, masked tokens are `{\em 2010}', `{\em Seattle}', `{\em Seahawks}', `{\em game}' and `{\em ,}' all of which found from the other sequence.
masked spans are `{\em 2010}', `{\em the Seattle Seahawks}' and `{\em to the}' all of which found from the other sequence. Note that a bigram `{\em game ,}' will not be able to masked out together, because although each of `{\em game}' and `{\em ,}' occurs in the other sequence, they do not co-occur together.
More implementation details are provided in Appendix~\ref{app:impl-details}.

\begin{figure*}[t]
\centering \footnotesize
\resizebox{2.05\columnwidth}{!}{\includegraphics{imgs/npminf-training.png}}
\caption{
The high-level idea of training \oursmulti\ (Section~\ref{subsubsec:ours-train-multi}).
\textcolor{orange}{\textbf{\mask\mask}} indicates the masked {\em span} whose target tokens are {\em the Seattle Seahawks}. 
%
We maximize the similarity scores between the first \mask\ and the start of the positive span, and between the second \mask\ and the end of the positive span.
%
%
% The high-level idea of training. \textbf{\ours\ (Section~\ref{subsec:ours}):} the similarity score between the masked token and tokens from other sequences with shared vocabulary is maximized using contrastive objective. \textbf{\oursmulti\ (Section~\ref{subsec:ours-multi}):} each masked \ngram\ is represented with two distinct \mask\ tokens and is subsequently mapped into two vectors: one for the start and the other for the end. We then maximize the similarity score between the first vector and the start of the co-occurring \ngram, as well as the second vector and the end of the co-occurring \ngram. \sewon{TODO: modify the figure}
}\label{fig:training-multi}
\end{figure*}


\subsection{\oursmulti}\label{subsec:ours-multi}

In typical encoder-only models, each \mask\ corresponds to one token, thus cannot be used when the number of tokens to predict is unknown.
For instance, in the third example of Figure~\ref{fig:intro}, {\em Thessaloniki} consists of 4 BPE tokens.
The existing encoder-only model is unable to predict it unless it knows in advance that the target entity consists of 4 BPE tokens, which is unrealistic.
We think this is a reason the encoder-only model has not been widely used in prompting, even though it generally outperforms the encoder-decoder or the decoder-only model in single-token prediction (which we show in Section~\ref{subsec:results-closed}).

To address this issue, we introduce \textbf{\oursmulti}, an extension of \ours\ that has an infinite output space by retrieving an \ngram\ to fill in a single \mask\ token.
Specifically, the encoder in \oursmulti\ represents a test query with two vectors, and use them to retrieve the start and the end of the span from the reference corpus.


\subsubsection{\oursmulti: Inference}\label{subsubsec:ours-inference-multi}
\oursmulti\ consists of the encoder and the corpus $\mathcal{C}$, and maps the text into a dense vector space as \ours\ does.
%
The difference from \ours\ is that at inference time, \oursmulti\ retrieves a {\em span} based on the score assigned to the {\em start} and the {\em end} assigned to the span.


Concretely, let $q_1...q_{t-1}, \mask, q_{t+1}...q_L$ be a query whose $t$-th token is \mask. We {\em duplicate} a \mask token, and form a sequence of $L+1$ tokens: $q_1...q_{t-1}, \mask, \mask, q_{t+1}...q_L$.
We then feed it into the encoder to obtain $L+1$ number of $h$-dimensional vectors, and take a vector corresponding to the first \mask\ and the second \mask\ as $\mathbf{q}^\mathrm{start}$ and $\mathbf{q}^\mathrm{end}$, respectively.
%
%$\mathbf{q}_1...\mathbf{q}_{L+1}$, and define $$ \mathbf{q}^\mathrm{start}=\mathbf{q}_t,\mathbf{q}^\mathrm{end}=\mathbf{q}_{t+1}.$$

\oursmulti\ uses $\mathbf{q}^\mathrm{start}$ and $\mathbf{q}^\mathrm{end}$ to find the start and the end of the \ngram\ to retrieve.
%
Intuitively, each distinct \ngram\ in the corpus $c_{i_1}...c_{i_n}$ is assigned a score $s(c_{i_1}...c_{i_n})$ defined as:$$\mathrm{exp}(\mathrm{sim}(\mathbf{q}^\mathrm{start},\mathbf{c}_{i_1}))+\mathrm{exp}(\mathrm{sim}(\mathbf{q}^\mathrm{end}, \mathbf{c}_{i_n})).$$
%
Finally, the prediction is made by aggregating these scores over possible candidates:$$\argmax_{v^* \in \mathcal{V}^*} \sum_{c^* \in \mathcal{C}^*}\mathbb{I}[v^*=c^*]s(c^*),$$ where $\mathcal{V}^*$ and $\mathcal{C}^*$ are sets of any possible \ngrams\ defined by the vocabulary $\mathcal{V}$ and the corpus $\mathcal{C}$, respectively. In practice, an approximation is made as in Section~\ref{subsubsec:ours-inference} which we detail in Appendix~\ref{app:impl-details}. 

\subsubsection{\oursmulti: Training}\label{subsubsec:ours-train-multi}
Training of \oursmulti\ largely follows training of \ours\ (Section~\ref{subsubsec:ours-train}) with a few key differences:
%
(1) we replace each distinct span with two \mask\ tokens,
%
(2) each distinct span has the start vector and the end vector, obtained from each of two \mask\ tokens, and
%
(3) we use the contrastive objective for the start and the end separately.

\vspace{-.2em}
\paragraph{Masking.}
We identified spans to mask out as done in Section~\ref{subsubsec:ours-train}.
%
Then, instead of replacing each token in the span with \mask, we replace the whole span with two \mask\ tokens. For instance, in Figure~\ref{fig:masking}, each of  `{\em 2010}', `{\em the Seattle Seahawks}' and `{\em to the}' is replaced with into `\mask\mask'.

\vspace{-.2em}
\paragraph{Key idea with an example.}
We illustrate an example in Figure~\ref{fig:training-multi}.
%
The masked span is {\em the Seattle Seahawks}, which we can find from another sequence in the batch.
%
We encourage the start vector of this masked span, i.e., the vector corresponding to the first \mask, to be closer to {\em the} of {\em Seattle Seahawks} while being distant from other tokens.
%
Note that it should not be any `{\em the}'; for instance, `{\em the}' of `{\em the first team in NFL history}' should still be encouraged to be distant from the start vector.
%
Similarly, we encourage the end vector of the masked span, i.e., the vector corresponding to the second \mask, to be closer to {\em Seahawks} of {\em the Seattle Seahawks} while being distant from other tokens.
%
This process is done to all masked spans regardless of the length of the span. For instance, if the span has a length of 1, e.g., {\em 2010} in the figure, then both the start vector and the end vector of the masked span are encouraged to be closer to the vector corresponding to {\em 2010}.

We formally define the training objective of \oursmulti\ in Appendix~\ref{app:ours-multi-objective}.


==> sections/07-discussion.tex <==
%We summarize broader implications, limitations, and future directions.

%\vspace{-.2em}
\paragraph{Scaling through the inference corpus.}
Parametric language models scale with the number of parameters and the number of tokens at training.
\Np\ models have a new dimension for scaling: the size of the reference corpus at inference time.
This is attractive since scaling can be done at inference without re-training the model.
In this paper, we scale the model up to nearly 1B tokens, but we think it is possible to scale further using tools such as Distributed FAISS~\citep{johnson2019billion} or ScaNN~\citep{avq_2020}.

\vspace{-.2em}
\paragraph{Complete removal of softmax enables a larger vocabulary.}
Large vocabulary is known to lead performance gains~\citep{conneau2020unsupervised} but is bounded in memory costs.
Previous work explored more efficient softmax approximations~\citep{morin2005hierarchical,chen2015strategies,pmlr-v70-grave17a}.
Our \np\ training offers an alternative by removing the softmax over the vocabulary.
With the RoBERTa architecture, increasing the vocab size by 2x makes the baseline training 50\% more memory expensive, but does not increase the memory in training \ours.
Future work can explore training \ours\ with a significantly larger vocabulary to further boost performance.

\vspace{-.2em}
\paragraph{Extension for generation.}
It is currently non-trivial to use \ours\ for generation, since it is the encoder-only model. Future work can explore autoregressive generation as done in \citet{patel2022bidirectional} or use \ours\ for editing~\citep{schick2022peer,gao2022attributed}.

\vspace{-.2em}
\paragraph{Extension to few-shot learning and fine-tuning.}
While our paper focuses on zero-shot evaluation, we think \ours\ is easy to extend to a few-shot learning setup. Fine-tuning \ours\ is significantly easier than fine-tuning larger models such as T5, OPT and GPT-3 which we compare \ours\ with, and can be explored in future work.

\vspace{-.2em}
\paragraph{Better cross-lingual transfer.}
Our models are able to predict extremely rare or unseen words by modeling a fully \np\ distribution.
%
This offers significant advantages in a multilingual setup.
%
\Np\ training may alleviate the burden of collecting large-scale multilingual corpora since it makes the model less sensitive to the language coverage in the training data, and may lead to significantly better cross-lingual transfer, as we demonstrate in the entity translation task.
%
We think future work can train multilingual \ours, and explore more comprehensive cross-lingual evaluation.

\vspace{-.2em}
\paragraph{Limitation in speed.}
We find that search makes inference considerably slower than the counterpart without search.
%
We think that (1) search can significantly be faster with better engineering (we use the default hyperparameters of the FAISS index with no tuning) or better index, and
(2) the speed of \ours\ is still on par with the speed of significantly larger parametric models that \ours\ outperforms.
%
Moreover, while not explored in this work, there has been work that improves inference speed~\citep{he-etal-2021-efficient,alon2022neuro} that can be applied to \ours.
%
We leave improving inference speed to future work.




==> sections/13-checklist.tex <==
%\paragraph{Potential Risk.}

\ours\ is a masked large language model that is pretrained on a text corpus including English Wikipedia and CC News, which potentially includes harmful and biased context, despite the original authors' best efforts to mine the text.
There are also potential risks in privacy and security if the data includes any personal information.
We thus highlight that \ours\ should be considered as a research prototype rather than a deployable system to real users, and continuing efforts are needed to reduce potential risks of the model.

==> sections/99-discard.tex <==

\begin{algorithm}
\caption{Clustering-based In-batch Training}\label{alg:clustering-in-batch-training}
\begin{algorithmic}[1] \small

\Procedure{Training\_step}{$\mathcal{B}$} % \Comment{This is one training step}
    \State\gitcomment{$N$: the number of sequences per GPU}
    \State\gitcomment{$L$: the number of tokens per sequence}
    \State\gitcomment{$M$: the number of GPUs}
    \State\gitcomment{$C$ is the number of clusters}
    \State $\mathcal{B}_1...\mathcal{B}_M \gets \mathrm{Split}(\mathcal{B}, M) $
    \For{$m \in [1, M]$ \gitcomment{Parallel}}
        \State $m$-th GPU computes $\mathbf{H}_{m} \in \mathbb{R}^{NL \times d}$
    \EndFor
    \State $\mathbf{H} \gets \mathrm{Concatenate}(\mathbf{H}_{1}...\mathbf{H}_{M}) \in \mathbb{R}^{MNL \times d}$
    \State $\mathbf{H}'_1...\mathbf{H}'_C \gets k\text{-means}(\mathbf{H})$
    \State $l \gets 0$ \gitcomment{Loss}
    \For{$c \in [1, C]$ \gitcomment{Parallel}}
        \State \gitcomment{each $\mathbf{H}'_c$ is handled by $\frac{M}{C}$ GPUs.}
        \State $\mathbf{H}'_{c,1}...\mathbf{H}'_{c,M/C } \gets \mathrm{Split}(\mathbf{H}'_c,\frac{M}{C} \}$
        \For{$m \in [1, \frac{M}{C}]$ \gitcomment{Parallel}}
            \State \gitcomment{$\left(\frac{M}{C}c + m\right)$-th GPU computes loss for}
            \State \gitcomment{$\mathbf{H}_{c,m}$ using $\mathbf{H}_c$ as a batch }
            \State $l \gets l + \mathrm{GetLoss}(\mathbf{H}_{c,m},\mathbf{H}_c)$ 
        \EndFor
    \EndFor
    \Return $l$
\EndProcedure

\end{algorithmic}
\end{algorithm}

\paragraph{Clustering-based in-batch training}
As the number of GPUs grows, the number of in-batch positives and negatives grows which may cause the memory error.\footnote{
    Let $M$ the number of GPUs, $N$ be the number of sequences in the batch per GPU, and $L$ be the number of tokens per sequence.
    The similarity matrix that one GPU should compute has a shape of $(N \times L, M \times N \times L)$.
    Therefore, as $M$ gets larger, the value of $N$ that one GPU can fit may decrease (assuming $L$ is fixed).
}
Instead of limiting the number of GPUs or the batch size, we use a subset of in-batch positives and negatives.
%
In particular, we re-distribute prefix representations in the entire batch based on their similarities, using $k$-means clustering.\footnote{
    Let the maximum size of the similarity matrix one GPU can handle be $(N \times L, \tilde{M} \times N \times L)$.
    We cluster $M \times N \times L$ vectors into $\ceil*{\frac{M}{\tilde{M}}}$ clusters.
}
%
Detail procedure is provided in Algorithm~\ref{alg:clustering-in-batch-training}.
%

This is based on the intuition that high-quality positives and negatives are those whose representations are similar---such positives are less likely to be false positives, and such negatives are more likely to be {\em hard} negatives.
Ablations in Section~\ref{subsec:ablations} show that this clustering-based method is critical in performance, compared to alternative such as randomly splitting the batch.
%





\subsection{\ours: Inference}

\subsection{Baselines}

We compare \ours\ and \ours+LM with a range of baselines. 
All models are trained with the same infrastructure (e.g., the number of GPUs, etc) and the same values of hyperparameters (e.g., batch size, the number of training steps, etc).

\vspace{.5em}
\noindent
\textbf{LM} is the standard LM.

\vspace{.3em}
\noindent
\textbf{LM\arrowbold\knnbold} uses the model trained with the standard LM objective, but uses the \knn\ at inference. This is equivalent to an extreme version of \citet{khandelwal2020generalization} and \citet{shi2022nearest} where the interpolation hyperparameter $\lambda$ is $0.0$.

\vspace{.3em}
\noindent
\textbf{LM\arrowbold{}\knnlmbold} uses the model trained with the standard LM objective, and uses the interpolation of the standard LM and \knn\ at inference. This is equivalent to \citet{khandelwal2020generalization} and \citet{shi2022nearest}. We follow them in using $\lambda=0.3$.

\vspace{.3em}
\noindent
\textbf{\ours\arrowbold{}LM} uses our trained model, \ours, and uses the standard LM at inference time with no retrieval. This is equivalent to \ours+LM with $\lambda=0$.

\vspace{.3em}
\noindent
\textbf{RA} is the model that is designed to be as close as possible as \citet{zhong2022training}, previous work that trains the LM with a retrieval component that supplements the standard LM objective.
The training objective is TODO.
The inference is same as \knnlm.
Differences from \citet{zhong2022training} include: (1) dropping the local and the long-term memory component,\footnote{This was motivated by the intuition that downstream tasks do not benefit much from the local and the long-term memory.} and (2) using our batching instead of the BM25 batching.\footnote{Their BM25-based batching was only possible because the training is in a relatively small scale; building the BM25 index over the pre-training corpus is not feasible.}
Note that \citet{zhong2022training} trains the model on the language modeling benchmark and does not scale it into a pre-training scale nor evaluated on downstream tasks---this baseline can be seen as the application of \citet{zhong2022training} for pre-training and downstream evaluation.

\vspace{.3em}
\noindent
\textbf{RA\arrowbold{}LM} takes the RA model and uses LM inference without any retrieval; this is equivalent to RA with $\lambda=0.0$.

\vspace{.3em}
\noindent
\textbf{RA\arrowbold{}\knnbold} takes the RA model and uses the retrieval component only; this is equivalent to RA with $\lambda=1.0$.

\begin{table}[t]
    \centering \footnotesize
    \begin{tabular}{l @{\hspace{0.8em}} l @{\hspace{0.2em}} r}
        \toprule
            Dataset & Task & $|\mathcal{C}|$ \\
        \midrule
            \multicolumn{3}{l}{\textbf{\em General tasks}} \\
            AGNews  & News topic classification     & 4\\
            Yahoo   & Question classification       & 10\\
            Subj    & Subjectivity classification   & 2\\
            SST-2   & Movie sentiment analysis      & 2\\
            MR      & Movie sentiment analysis      & 2\\
            RT      & Movie sentiment analysis      & 2\\
            CR      & Customer sentiment analysis   & 2\\
            Amazon  & Product sentiment analysis    & 2\\
        \midrule
            \multicolumn{3}{l}{\textbf{\em Knowledge-dependent tasks}} \\
            LAMA T-REx       & Knowledge probing & -\\
            LAMA Google RE   & Knowledge probing & -\\
            KAMEL            & Knowledge probing/Question answering & - \\
            NQ               & Question answering & -\\
            TriviaQA         & Question answering & -\\
        \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
        A list of downstream tasks used in the experiments.
    }\label{tab:datasets}
\end{table}


\begin{table*}[t]
    \centering \scriptsize
    \begin{tabular}{l @{\hspace{-0.2em}} r @{\hspace{2em}}  rrrrrrrrrr}
        \toprule
            \multirow{2}{*}{Model} & \multirow{2}{*}{\#Params} & \multicolumn{3}{c}{T-REx} & \multicolumn{2}{c}{G-RE Long} &
            \multicolumn{2}{c}{G-RE Short} &\multirow{2}{*}{KML} & \multirow{2}{*}{TQA} & \multirow{2}{*}{NQ} \\
            \cmidrule(lr){3-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
            && All & UHN & Hard & All & UHN & All & UHN \\
        \midrule
            \multicolumn{6}{l}{\textbf{\em Baselines (encoder-decoder)}} \\
            T5          & 2.2x & 13.3 (15.3) & 5.5 (6.0) & 10.7 (12.6) & 12.5 (14.3) & 8.2 (9.3) & 1.1 (1.2) & 0.4 (0.4) & 1.6 (1.8) & 4.2 (4.4) & 0.5 (0.8)\\
            ~~~~+ BM25  & 2.2x & 22.2 (34.2) & 20.3 (29.7) & 22.4 (33.9) & 47.3 (54.3) & 48.5 (54.2) & 16.4 (34.3) & 16.6 (33.5) & 13.9 (16.4) & 31.4 (34.6) & 5.2 (6.3) \\
            T5 3B       & 8.5x & 12.1 (13.1) & 8.2 (8.6) & 11.5 (12.3) & 16.2 (18.6) & 12.0 (13.0) & 2.1 (2.2) & 0.7 (0.7) & 3.6 (3.9) & 9.0 (9.9) & 2.0 (2.4) \\
            ~~~~+ BM25  & 8.5x & 21.6 (36.0) & 19.0 (31.2) & 21.8 (35.5) & 52.7 (59.4) & 53.1 (58.7) & 18.5 (40.7) & 15.5 (39.4) & 16.2 (22.0) & 39.6 (43.2) & 10.8 (13.1) \\
        \midrule
            \multicolumn{6}{l}{\textbf{\em Baselines (decoder-only)}} \\
            GPT-3 2.7B  & 7.6x  &&&&&&&& 0.0 (0.1) & 0.1 (0.3) & 0.1 (0.3) \\
            ~~~~+ BM25  & 7.6x  &&&&&&&& 1.4 (5.9) & 4.2 (12.9) & 2.0 (6.3) \\
            GPT-3 6.7B  & 19x   &&&&&&&& 0.5 (4.2) & 4.8 (15.9) & 1.4 (6.9) \\
            ~~~~+ BM25  & 19x   &&&&&&&& 1.0 (7.8) & 5.7 (19.2) & 3.1 (11.0) \\
            GPT-3 13B   & 37x   &&&&&&&& 0.8 (3.6) & 7.8 (16.3) & 2.8 (9.4) \\
            ~~~~+ BM25  & 37x   &&&&&&&& 3.7 (12.2) & 13.3 (25.2) & 5.0 (13.4) \\
            GPT-3 175B  & 500x  &&&&&&&& 4.9 (13.7) & 39.6 (51.6) & 10.2 (25.3) \\
            ~~~~+ BM25  & 500x  &&&&&&&& 9.0 (28.7) & 35.7 (54.8) & 4.4 (27.0) \\
        \midrule
            \multicolumn{6}{l}{\textbf{\em Ours (encoder-only, nonparametric)}} \\
            \oursmulti      & 1.0x & \\
            ~~~~+ BM25 Top 3 & 1.0x & xx.x & xx.x & xx.x & 42.7 & 41.8 & 27.8 & 22.8 & 15.9 & xx.x & xx.x \\
            ~~~~+ BM25 Top 100 & 1.0x & 30.6 & 23.2 & 28.7 & 30.9 & 26.5 & 13.9 & 8.4 & 10.0 & 28.1 & 10.9 \\
        \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
        Results on open-set tasks.
        {\em \# Params} indicates the relative number of model parameters compared to RoBERTa large (354M). RoBERTa, T5 and GPT-2 are their {\em large} variants unless specified otherwise.
        For LAMA (T-REx, G-RE Long and G-RE Short), the macro-average over 1, 2, 3 and 4+ grams are reported.
        All models are zero-shot.
        See Table~\ref{tab:comparison-to-gpt3} for comparisons with GPT-3 zero-shot and few-shot.
    }\label{tab:open-set}
\end{table*}

\begin{table*}[t]
    \centering \scriptsize
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l @{\hspace{-0.2em}} rc @{\hspace{2em}}  rrrrrrrr}
        \toprule
            \multirow{2}{*}{Model} & \multirow{2}{*}{\#Params} & \multirow{2}{*}{$\mathcal{C}$} & \multicolumn{3}{c}{T-REx} & 
            \multicolumn{2}{c}{Google RE} &\multirow{2}{*}{KML} & \multirow{2}{*}{TQA} & \multirow{2}{*}{NQ} \\
            \cmidrule(lr){4-6} \cmidrule(lr){7-8}
            &&& All & UHN & Hard & All & UHN \\
        \midrule
            \multicolumn{6}{l}{\textbf{\em Baselines (encoder-decoder)}} \\
            T5          & 2.2x && 13.3 (15.3) & 5.5 (6.0) & 10.7 (12.6) & 1.1 (1.2) & 0.4 (0.4) & 1.6 (1.8) & 4.2 (4.4) & 0.5 (0.8)\\
            T5 3B       & 8.5x && 12.1 (13.1) & 8.2 (8.6) & 11.5 (12.3) & 2.1 (2.2) & 0.7 (0.7) & 3.6 (3.9) & 9.0 (9.9) & 2.0 (2.4) \\
        \cmidrule(lr){1-11}
            BM25 + T5 & 2.2x & \checkmark & 22.2 (34.2) & 20.3 (29.7) & 22.4 (33.9) & 16.4 (34.3) & 16.6 (33.5) & 13.9 (16.4) & 31.4 (34.6) & 5.2 (6.3) \\
            BM25 + T5 3B & 8.5x & \checkmark & 21.6 (36.0) & 19.0 (31.2) & 21.8 (35.5) & 18.5 (40.7) & 15.5 (39.4) & \textbf{16.2} (22.0) & 39.6 (43.2) & 10.8 (13.1) \\
        \midrule
            \multicolumn{6}{l}{\textbf{\em Baselines (decoder-only)}} \\
            OPT 2.7B  & 7.6x& & 9.8 (13.9) & 6.7 (7.5) & 8.3 (11.4) & 0.0 (0.1) & 0.0 (0.0) & 1.6 (11.4) & 9.9 (26.3) & 2.1 (8.4) \\
            GPT-3 2.7B  & 7.6x  && 4.4 (10.0) & 2.6 (3.3) & 3.8 (7.6) & 0.0 (0.1) & 0.0 (0.0) & 2.1 (5.3) & 5.2 (11.8) & 1.1 (3.3) \\
            OPT 6.7B  & 19x& & 11.6 (15.9) & 9.9 (11.1) & 10.7 (14.8) & 0.6 (1.3) & 0.3 (0.4) & 3.2 (12.9) & 20.9 (36.7) & 4.2 (14.7) \\
            GPT-3 6.7B  & 19x   && 8.1 (10.3) & 5.0 (5.6) & 6.7 (8.6) & 0.0 (0.0) & 0.0 (0.0) & 2.1 (8.7) & 12.4 (24.4) & 3.1 (7.9) \\
            OPT 13B  & 37x & & 15.0 (20.6) & 12.7 (14.5) & 12.7 (18.0) & 0.3 (0.6) & 0.3 (0.4) & 2.5 (14.0) & 22.5 (40.2) & 4.2 (13.9) \\
            GPT-3 13B   & 37x   && 16.4 (22.6) & 13.7 (16.1) & 15.5 (20.2) & 0.8 (1.1) & 0.4 (0.7) & 2.2 (12.8) & 25.5 (41.1) & 5.2 (13.4) \\
            GPT-3 175B  & 500x  && 25.7 (36.9) & 24.1 (31.1) & 24.7 (34.7) & 1.1 (2.1) & 1.0 (1.7) & 6.5 (19.2) & \textbf{49.0} (62.2) & \textbf{11.4} (26.5) \\
        \cmidrule(lr){1-11}
            BM25 + OPT 2.7B  & 7.6x& \checkmark & 14.8 (34.5) & 14.1 (25.4) & 13.8 (30.9) & 4.4 (22.2) & 3.7 (22.0) & 11.3 (29.8) & 28.5 (48.6) & 8.3 (22.4) \\
            BM25 + GPT-3 2.7B & 7.6x  & \checkmark & 3.5 (21.9) & 3.4 (15.0) & 3.6 (20.4) & 0.1 (9.8) & 0.1 (10.8) & 5.2 (21.5) & 14.5 (36.4) & 6.1 (14.2) \\
            BM25 + OPT 6.7B  & 19x& \checkmark & 14.8 (32.4) & 14.3 (27.3) & 14.9 (31.2) & 4.1 (22.6) & 3.3 (21.6) & 8.2 (32.7) & 29.9 (56.2) & 10.7 (26.8) \\
            BM25 + GPT-3 6.7B & 19x   & \checkmark & 14.9 (25.4) & 15.3 (20.2) & 15.1 (23.9) & 4.4 (11.8) & 3.5 (11.5) & 7.0 (26.3) & 21.1 (45.6) & 8.8 (18.0) \\
            BM25 + OPT 13B  & 37x & \checkmark & 18.9 (36.3) & 19.1 (31.1) & 19.3 (34.9) & 3.8 (24.1) & 3.1 (24.4) & 10.6 (33.7) & 34.0 (57.1) & 10.7 (27.5) \\
            BM25 + GPT-3 13B & 37x   & \checkmark & 22.2 (40.1) & 22.7 (34.1) & 22.4 (37.9) & 11.8 (33.8) & 11.2 (34.3) & 8.9 (31.2) & 32.4 (55.7) & 11.2 (26.7) \\
            BM25 + GPT-3 175B & 500x  & \checkmark & 32.0 (48.1) & \textbf{31.6} (44.1) & 31.3 (46.7) & 11.4 (34.5) & 11.9 (35.5) & 12.2 (36.9) & 44.9 (68.3) & 6.4 (37.0) \\
        \midrule
            \multicolumn{6}{l}{\textbf{\em Ours (encoder-only, nonparametric)}} \\
            \oursmulti      & 1.0x & \checkmark & 16.1 & 11.9 & 14.4 & \\
            ~~~~with Sparse & 1.0x & \checkmark & \textbf{34.5} & 29.0 & \textbf{32.1} & \textbf{27.9} & \textbf{23.0} & 15.6 & 32.2 & 10.8 \\
            %~~~~with Sparse & 1.0x & \checkmark & 34.6 & 28.8 & 32.5 & 27.8 & 22.8 & 15.9 & 33.2 & 10.9 \\ [outdated numbers]
            %~~~~with Sparse & 1.0x & \checkmark & 30.6 & 23.2 & 28.7 & 13.9 & 8.4 & 10.0 & 28.1 & 10.9 \\ [outdated numbers]
        \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
        Results on open-set tasks.
        {\em \# Params} indicates the relative number of model parameters compared to RoBERTa large (354M), and $\mathcal{C}$ indicates whether a text corpus is used.
        For LAMA (T-REx and Google RE), the macro-average over 1, 2, 3 and 4+ grams are reported.
        All models are zero-shot.
    }\label{tab:open-set}
\end{table*}


\begin{table*}[t]
    \centering \footnotesize
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l @{\hspace{-0.5em}} r @{\hspace{1em}} c @{\hspace{1em}} rr rr a}
        \toprule
            \multirow{2}{*}{Model} & \multirow{2}{*}{\#Params} & \multirow{2}{*}{$\mathcal{C}$} & \multicolumn{2}{c}{\em Unchanged} & 
            \multicolumn{2}{c}{\em Changed} & {AVG}\\
            \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
            &&& 2019 & 2022 & 2019 & 2022 & 2022\\
        \midrule
            \multicolumn{7}{l}{\textbf{\em Baselines (encoder-decoder)}} \\
            T5          & 2.2x && \multicolumn{2}{c}{0.4 (0.8)} & \multicolumn{2}{c}{1.9 (2.5)} & 1.1 (1.6) \\
            T5 3B       & 8.5x && \multicolumn{2}{c}{0.4 (0.6) } & \multicolumn{2}{c}{1.8 (2.0) } & 1.1 (1.3) \\
        \cmidrule(lr){1-7}
            BM25 + T5 & 2.2x & \checkmark & 3.0 (4.7) & \textbf{20.1} (29.5) & 13.7 (24.6) & 14.9 (26.3) & 17.5 (27.9) \\
            BM25 + T5 3B & 8.5x & \checkmark & 2.2 (4.5) & 17.8 (27.9) & 11.9 (23.1) & 12.0 (23.2) & 14.9 (25.5) \\
        \midrule
            \multicolumn{7}{l}{\textbf{\em Baselines (decoder-only)}} \\
            OPT 6.7B        & 19x   && \multicolumn{2}{c}{1.0 (1.5)} & \multicolumn{2}{c}{2.5 (3.2)} & 1.7 (2.3)\\
            OPT 13B         & 37x   && \multicolumn{2}{c}{2.1 (2.5)} & \multicolumn{2}{c}{4.9 (6.1)} & 3.5 (4.3) \\
        \cmidrule(lr){1-7}
            BM25 + OPT 6.7B        & 19x & \checkmark & 1.7 (4.6) & 11.3 (16.8) & 10.2 (18.0) & 8.2 (13.7) & 9.7 (15.2) \\
            BM25 + OPT 13B         & 37x & \checkmark & 2.8 (5.3) & 16.6 (24.2) & 14.8 (23.4) & 14.4 (22.9) & 15.5 (23.5) \\
        \midrule
            \multicolumn{7}{l}{\textbf{\em Ours (encoder-only, nonparametric)}} \\
            \oursmulti  & 1.0x & \checkmark & - & - & - & - \\
            ~~~~with Sparse  & 1.0x & \checkmark & 18.9 & 19.5 & 2.9 & \textbf{17.5} & \textbf{18.5} \\
        \bottomrule
    \end{tabular}\vspace{-.1em}
    \caption{
        Results on \templama.
        {\em \# Params} indicates the relative number of model parameters compared to RoBERTa large (354M), and $\mathcal{C}$ indicates whether a text corpus is used.
    }\label{tab:temporal-open-set}
\end{table*}



